FlexER: Flexible Entity Resolution for Multiple Intents

Entity resolution, a longstanding problem of data cleaning and integration, aims at identifying data records that represent the same real-world entity. Existing approaches treat entity resolution as a universal task, assuming the existence of a single interpretation of a real-world entity and focusing only on finding matched records, separating corresponding from non-corresponding ones, with respect to this single interpretation. However, in real-world scenarios, where entity resolution is part of a more general data project, downstream applications may have varying interpretations of real-world entities relating, for example, to various user needs. In what follows, we introduce the problem of multiple intents entity resolution (MIER), an extension to the universal (single intent) entity resolution task. As a solution, we propose FlexER, utilizing contemporary solutions to universal entity resolution tasks to solve multiple intents entity resolution. FlexER addresses the problem as a multi-label classification problem. It combines intent-based representations of tuple pairs using a multiplex graph representation that serves as an input to a graph neural network (GNN). FlexER learns intent representations and improves the outcome to multiple resolution problems. A large-scale empirical evaluation introduces a new benchmark and, using also two well-known benchmarks, shows that FlexER effectively solves the MIER problem and outperforms the state-of-the-art for a universal entity resolution.

==> results3.tex <==
%\subsection{Intents Ablation study}\label{sec:ablation}
%\bg{TBC}

\subsection{Intra-Layer Edges Contribution}\label{sec:intra-edges}
\bg{TBC}



==> results4.tex <==

\subsection{Run-Time Complexity Analysis}\label{sec:comlexity}
\bg{TBC}


%\begin{figure*}[t]
%	\centering
%	\begin{subfigure}[b]{0.24\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figs/HMamazon}
%		\caption{AmazonMI}
%		\label{fig:HMamazom}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.24\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figs/HMitune}
%		\caption{iTunes-Amazon}
%		\label{fig:HMitunes}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.24\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figs/HMwalmart}
%		\caption{Walmart-Amazon}
%		\label{fig:HMwalmart}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.24\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figs/HMWDC}
%		\caption{WDC}
%		\label{fig:HMWDC}
%	\end{subfigure}
%	\caption{Correlation between the likelihood scores for the different intents of each dataset}
%	\label{fig:HMintents}
%\end{figure*}
%
%As a final analysis, we look into the relationships between intents. Recall that the edge weights for training the GCN are computed over the training set (see Section~\ref{sec:Gcreate}). To allow a better examination of the results, we use the correlation (Eq.~\ref{eq:corr}) between the likelihood scores (a value in $[0,1]$ that when accompanied with a threshold provides a binary classification) of the different single-intent models over the test set. Specifically, Figure~\ref{fig:HMintents} presents a heatmap for each dataset to illustrates the correlation between intent pairs.
%
%Recall that for the tested datasets, all intents overlap (see Definition~\ref{def:overlap}). Therefore, the intent graph is a complete graph with edges between every two nodes. Examining Figure~\ref{fig:HMintents}, we observe that the predictions for some intents are very correlated (\emph{e.g.,} {\em Brand} and {\em Eq.} for the AmazonMI, Figure~\ref{fig:HMamazom}) and for some are not at all (\emph{e.g.,} {\em Genre} and {\em Artist} for the iTunes-Amazon, Figure~\ref{fig:HMitunes}). This possibly suggests that even when two intents overlap they may still have (very) different ``opinions'' regarding record pairs. 
%
%Looking at the equivalence intent ({\em Eq.}), representing the focus of research so far, we observe that it is only weakly related to some intents. For example, for the Walmart-Amazon dataset, {\em Eq.} is very weakly related to {\em Price} (0.075) and only weakly related to {\em Brand+Price} (0.14). This means that when providing a ``standard'', universal-based solution for a user seeking to group together products that share the same brand and price range would fail to satisfy her needs. 
%In addition, looking at composed intents, we observe that 

%\ag{perhaps add some more discussion points. For example, the following three points: 1. Eq., which was the focus of research so far, is only weakly related to some intents, e.g., for the Walmart-Amazon dataset, Eq. is very weakly related to Price (0.075). 2) a combined intent (like category-set+Main category may have a weaker impact to one of its components, e.g., Main-category (0.43), than to other intents, e.g., Brand (0.56). 3) Also, combined intents have veraying impacts on their components, e.g., Brand+Price with Brand (0.79) and Price (0.56)}
